ALIGNet: Partial-Shape Agnostic Alignment via Unsupervised Learning

The process of aligning a pair of shapes is a fundamental operation in computer graphics. Traditional approaches rely heavily on matching corresponding points or features to guide the alignment, a paradigm that falters when significant shape portions are missing. These techniques generally do not incorporate prior knowledge about expected shape characteristics, which can help compensate for any misleading cues left by inaccuracies exhibited in the input shapes. We present an approach based on a deep neural network, leveraging shape datasets to learn a shape-aware prior for source-to-target alignment that is robust to shape incompleteness. In the absence of ground truth alignments for supervision, we train a network on the task of shape alignment using incomplete shapes generated from full shapes for self-supervision. Our network, called ALIGNet, is trained to warp complete source shapes to incomplete targets, as if the target shapes were complete, thus essentially rendering the alignment partial-shape agnostic. We aim for the network to develop specialized expertise over the common characteristics of the shapes in each dataset, thereby achieving a higher-level understanding of the expected shape space to which a local approach would be oblivious. We constrain ALIGNet through an anisotropic total variation identity regularization to promote piecewise smooth deformation fields, facilitating both partial-shape agnosticism and post-deformation applications. We demonstrate that ALIGNet learns to align geometrically distinct shapes, and is able to infer plausible mappings even when the target shape is significantly incomplete. We show that our network learns the common expected characteristics of shape collections, without over-fitting or memorization, enabling it to produce plausible deformations on unseen data during test time.

==> figures/HoF/figure.tex <==
\begin{figure*}[h]
\newcommand{\hoffig}{2.3}
\begin{tabular}{ c  c  c | c  c  c }

% airplane
\includegraphics[width=\hoffig cm]{figures/HoF/airplane6/sample019_source.png} &
\includegraphics[width=\hoffig cm]{figures/HoF/airplane6/sample019_target.png} & 
\includegraphics[width=\hoffig cm]{figures/HoF/airplane6/sample019_targetPred.png} &
% airplane
\includegraphics[width=\hoffig cm]{figures/HoF/airplane7/sample001_source.png} &
\includegraphics[width=\hoffig cm]{figures/HoF/airplane7/sample003_target.png} &
\includegraphics[width=\hoffig cm]{figures/HoF/airplane7/sample003_targetPred.png} \\
\hline

% pear
\includegraphics[width=\hoffig cm]{figures/HoF/pear4/sample006_source.png} &
\includegraphics[width=\hoffig cm]{figures/HoF/pear4/sample006_target.png} & 
\includegraphics[width=\hoffig cm]{figures/HoF/pear4/sample006_targetPred.png} &
% bat
\includegraphics[width=\hoffig cm]{figures/HoF/bat2_airplane/sample005_source.png} &
\includegraphics[width=\hoffig cm]{figures/HoF/bat2_airplane/sample005_target.png} &
\includegraphics[width=\hoffig cm]{figures/HoF/bat2_airplane/sample005_targetPred.png} \\
\hline

% caption
source &
target & 
warped &
source &
target &
warped \\
\end{tabular}
\caption{More \ourmethod{} results. Triplets of: source, target and warped result.}
\label{fig:HoF}
\end{figure*}

==> figures/ablation/reg_table.tex <==
\begin{table}
\center
\csvautotabular{figures/ablation/vessel/table.csv}
\csvautotabular{figures/ablation/bottle/table.csv}
\csvautotabular{figures/ablation/vase/table.csv}
\csvautotabular{figures/ablation/airplane/table.csv}
\caption{Quantitative comparison for }
\label{table:reg}
\end{table}

==> figures/bird_figure/figure.tex <==
\begin{figure}
% partial targets
\jsubfig{}{}%
    \hfill \jsubfig{\includegraphics[height=1.6cm]{figures/birds/birds1/sample002_target.png}}
	%{(b) }%
    \hfill \jsubfig{\includegraphics[height=1.6cm]{figures/birds/birds1/sample005_target.png}}
	%{(c) }%
    \hfill \jsubfig{\includegraphics[height=1.6cm]{figures/birds/birds1/sample007_target.png}}
	%{(d) }%
    \hfill  \jsubfig{\includegraphics[height=1.6cm]{figures/birds/birds1/sample023_target.png}}
    { }%
    
% source1 & warps1    
    \jsubfig{\includegraphics[height=1.6cm]{{figures/birds/birds1/sample001_source.png}}}
	{}%
    \hfill \jsubfig{\includegraphics[height=1.6cm]{figures/birds/birds1/sample002_targetPred.png}}
	%{(b) }%
    \hfill \jsubfig{\includegraphics[height=1.6cm]{figures/birds/birds1/sample005_targetPred.png}}
	%{(c) }%
    \hfill \jsubfig{\includegraphics[height=1.6cm]{figures/birds/birds1/sample007_targetPred.png}}
	%{(d) }%
    \hfill  \jsubfig{\includegraphics[height=1.6cm]{figures/birds/birds1/sample023_targetPred.png}}
    { }%
    
% source2 & warps2    
    \jsubfig{\includegraphics[height=1.6cm]{{figures/birds/birds3/sample001_source.png}}}
	{}%
    \hfill \jsubfig{\includegraphics[height=1.6cm]{figures/birds/birds3/sample002_targetPred.png}}
	%{(b) }%
    \hfill \jsubfig{\includegraphics[height=1.6cm]{figures/birds/birds3/sample005_targetPred.png}}
	%{(c) }%
    \hfill \jsubfig{\includegraphics[height=1.6cm]{figures/birds/birds3/sample007_targetPred.png}}
	%{(d) }%
    \hfill  \jsubfig{\includegraphics[height=1.6cm]{figures/birds/birds3/sample023_targetPred.png}}
    { }%
    
\caption{Transferring source bird texture to different partial target airplanes.  }
\label{fig:bird_airplane_textures}

\end{figure}



%\begin{comment}
\begin{figure}
% partial targets
\jsubfig{}{}%
    \hfill \jsubfig{\includegraphics[height=1.6cm]{figures/airplanes/airplanes7/sample002_target.png}}
	%{(b) }%
    \hfill \jsubfig{\includegraphics[height=1.6cm]{figures/airplanes/airplanes7/sample001_target.png}}
	%{(c) }%
    \hfill \jsubfig{\includegraphics[height=1.6cm]{figures/airplanes/airplanes7/sample003_target.png}}
	%{(d) }%
    \hfill  \jsubfig{\includegraphics[height=1.6cm]{figures/airplanes/airplanes7/sample022_target.png}}
    { }%
    
% source1 & warps1    
    \jsubfig{\includegraphics[height=1.6cm]{{figures/airplanes/airplanes7/sample001_source.png}}}
	{}%
    \hfill \jsubfig{\includegraphics[height=1.6cm]{figures/airplanes/airplanes7/sample002_targetPred.png}}
	%{(b) }%
    \hfill \jsubfig{\includegraphics[height=1.6cm]{figures/airplanes/airplanes7/sample001_targetPred.png}}
	%{(c) }%
    \hfill \jsubfig{\includegraphics[height=1.6cm]{figures/airplanes/airplanes7/sample003_targetPred.png}}
	%{(d) }%
    \hfill  \jsubfig{\includegraphics[height=1.6cm]{figures/airplanes/airplanes7/sample022_targetPred.png}}
    { }%
    
% source2 & warps2    
    \jsubfig{\includegraphics[height=1.6cm]{{figures/airplanes/airplanes8/sample001_source.png}}}
	{}%
    \hfill \jsubfig{\includegraphics[height=1.6cm]{figures/airplanes/airplanes8/sample002_targetPred.png}}
	%{(b) }%
    \hfill \jsubfig{\includegraphics[height=1.6cm]{figures/airplanes/airplanes8/sample001_targetPred.png}}
	%{(c) }%
    \hfill \jsubfig{\includegraphics[height=1.6cm]{figures/airplanes/airplanes8/sample003_targetPred.png}}
	%{(d) }%
    \hfill  \jsubfig{\includegraphics[height=1.6cm]{figures/airplanes/airplanes8/sample022_targetPred.png}}
    { }%

% source3 & warps3    
    \jsubfig{\includegraphics[height=1.6cm]{{figures/airplanes/airplanes5/sample001_source.png}}}
	{Source}%
    \hfill \jsubfig{\includegraphics[height=1.6cm]{figures/airplanes/airplanes5/sample002_targetPred.png}}
	%{(b) }%
    \hfill \jsubfig{\includegraphics[height=1.6cm]{figures/airplanes/airplanes5/sample001_targetPred.png}}
	%{(c) }%
    \hfill \jsubfig{\includegraphics[height=1.6cm]{figures/airplanes/airplanes5/sample003_targetPred.png}}
	%{(d) }%
    \hfill  \jsubfig{\includegraphics[height=1.6cm]{figures/airplanes/airplanes5/sample022_targetPred.png}}
    { }%    
\caption{Transferring source texture to different partial target shapes.  }
\label{fig:airplane_textures}

\end{figure}
%\end{comment}

==> figures/complex_part/figure.tex <==
\begin{comment}
vessel: 389
\end{comment}

\begin{figure}[h]
\newcommand{\cmplx}{1.6}

% airplane
    \jsubfig{{\hspace*{\cmplx cm}}} {}  %
    \hfill \jsubfig{\includegraphics[width=\cmplx cm]{figures/complex_part/airplane/sample036_target.png}} {}%
    \hfill \jsubfig{\includegraphics[width=\cmplx cm]{figures/complex_part/airplane/sample040_target.png}} {}%
    \hfill \jsubfig{\includegraphics[width=\cmplx cm]{figures/complex_part/airplane/sample052_target.png}} {}%
    \hfill \jsubfig{\includegraphics[width=\cmplx cm]{figures/complex_part/airplane/sample055_target.png}} {}%

    \jsubfig{\includegraphics[width=\cmplx cm]{{figures/complex_part/airplane/sample036_source.png}}} {}%
    \hfill \jsubfig{\includegraphics[width=\cmplx cm]{figures/complex_part/airplane/sample036_targetPred.png}} {}%
    \hfill \jsubfig{\includegraphics[width=\cmplx cm]{figures/complex_part/airplane/sample040_targetPred.png}} {}%
    \hfill \jsubfig{\includegraphics[width=\cmplx cm]{figures/complex_part/airplane/sample052_targetPred.png}} {}%
    \hfill \jsubfig{\includegraphics[width=\cmplx cm]{figures/complex_part/airplane/sample055_targetPred.png}} {}%
    

    

    
    
\caption{Example results with complex, non-rectangular missing parts.}
\label{fig:complex_part}
\end{figure}

==> figures/grot/figure.tex <==
%/home/rana/dan3/silhouettes/rendered/airplane/checkpoint/alignet_2d_globalR,RRng=-0.5..0.5,augmentAffine=t,batchSize=200,cage_reg=1e-05,delCage=t,global_r=t,pWinSz1=20,pWinSz2=20,winsize_file=sz2020/SatMar3102:53:222018/

\begin{figure}[h]
\newcommand{\rotfig}{1.5}
\setlength\tabcolsep{3pt}
\begin{tabular}{c c c c c}

\includegraphics[width=\rotfig cm]{figures/grot/airplane/sample787_source.png} &
%\includegraphics[width=\rotfig cm]{figures/grot/airplane/sample787_target.png} &
\includegraphics[width=\rotfig cm]{figures/grot/airplane/sample790_target.png} &
%\includegraphics[width=\rotfig cm]{figures/grot/airplane/sample791_target.png} &
\includegraphics[width=\rotfig cm]{figures/grot/airplane/sample801_target.png} &
\includegraphics[width=\rotfig cm]{figures/grot/airplane/sample802_target.png} &
%\includegraphics[width=\rotfig cm]{figures/grot/airplane/sample806_target.png} &
\includegraphics[width=\rotfig cm]{figures/grot/airplane/sample807_target.png} \\

 &
%\includegraphics[width=\rotfig cm]{figures/grot/airplane/sample787_targetPred.png} &
\includegraphics[width=\rotfig cm]{figures/grot/airplane/sample790_targetPred.png} &
%\includegraphics[width=\rotfig cm]{figures/grot/airplane/sample791_targetPred.png} &
\includegraphics[width=\rotfig cm]{figures/grot/airplane/sample801_targetPred.png} &
\includegraphics[width=\rotfig cm]{figures/grot/airplane/sample802_targetPred.png} &
%\includegraphics[width=\rotfig cm]{figures/grot/airplane/sample806_targetPred.png} &
\includegraphics[width=\rotfig cm]{figures/grot/airplane/sample807_targetPred.png} \\

%% &
%a &
%%b &
%c &
%%d &
%%e &
%f &
%%g \\

\end{tabular}
\caption{\new{Incorporation of unsupervised arbitrary global orientation estimation. Training and testing on offsets 
in the range $[-30,30]$.}}
%of $\pm 30^{\circ}$}. }
\label{fig:grot}
\end{figure}

==> figures/grot/table.tex <==
\begin{table}
\begin{center}
\begin{tabular}{c || c || c|} 
%\hline
%\multicolumn{2}{c}{2D} \\
orientation estimation & 2D & 3D \\
\hline
without & \td{x} & \td{x} \\ [0.2ex] 
\hline
with & \td{x} & \td{x} \\ [0.2ex] 
%\hline\hline\hline\hline
\end{tabular}
\end{center}
\caption{\revb{Quantitative global orientation results on rotated partial \emph{airplanes} test set. Training on rotated shapes \emph{without} (top) and \emph{with} (bottom) adding global orientation estimation. Rotational offsets are uniformly sampled in the range of $[-30^{\circ},30^{\circ}]$ (as shown in Figure~\ref{fig:grot}). Displayed: test accuracy results of \ourmethod{} with and without incorporation of global orientation estimation (bottom and top, respectively).}}
\label{tab:grot}
\end{table}


%Incorporating orientation estimation handles rotated shapes better in 2D and 3D.

==> figures/limitations/class_sp_fig.tex <==
\begin{figure}[h]
\newcommand{\limfig}{1.1}
\setlength\tabcolsep{5pt} % default value: 6pt
\begin{tabular}{c c c c c c}

%\overbrace{}^\text{complex number}

%\multicolumn{2}{c}{\overbrace{}^\text{Input Class:}} &
%\multicolumn{4}{c}{\textbf{Trained Class:} } \

%\multicolumn{2}{c}{\textbf{Input Class:}} &
%\multicolumn{4}{c}{\textbf{Trained Class:} } \\

\multicolumn{2}{c}{$\overbrace{\rule{2.6cm}{0pt}}^\text{Input Class}$} &
\multicolumn{4}{c}{$\overbrace{\rule{5.5cm}{0pt}}^\text{Trained Class}$} \\

\multicolumn{2}{c}{\textit{airplane}} &
\textit{airplane} &
\textit{vessel} &
\textit{vase} & 
\textit{guitar} \\

\includegraphics[height=\limfig cm]{figures/limitations/airplanes_boat/sample027_source.png} &
\includegraphics[height=\limfig cm]{figures/limitations/airplanes_boat/sample027_target.png} &
\includegraphics[height=\limfig cm]{figures/limitations/airplanes_boat/sample027_targetPred.png} &
\includegraphics[height=\limfig cm]{figures/limitations/airplanes_boat/sample027_targetPred_vessel.png} &
\includegraphics[height=\limfig cm]{figures/limitations/airplanes_vase/sample027_targetPred.png} &
\includegraphics[height=\limfig cm]{figures/limitations/airplane_guitar/sample027_targetPred.png} \\

source &
target &
 &
 &
 & 
 \\
 \end{tabular}
\caption{Limitations of a class specific network. \ourmethod{} learns the essence of the shape collection it is trained on, which does not result in generalization on geometrically divergent classes.}
\label{fig:limitations}
\end{figure}



\begin{comment}

 Orientation estimation: FFDnet learns from the data, therefore absent rotations in a collection (\emph{e.g.,} airplane set) orientation is not able to be correctly estimated. However, classes which contain rotations (\emph{e.g.,} guitars) are indeed able to recover orientation deviations similar to the dataset.

 \\[0.5cm]
 
 \hline
 \hline
 
  \\[0.5cm]

\end{tabular}

\begin{tabular}{c c c  | c c c}

\multicolumn{3}{c}{Dataset with rotations} &
\multicolumn{3}{c}{Dataset without rotations} \\

\includegraphics[height=\limfig cm]{figures/limitations/guitar_rotation/sample019_source.png} &
\includegraphics[height=\limfig cm]{figures/limitations/guitar_rotation/sample019_target.png} &
\includegraphics[height=\limfig cm]{figures/limitations/guitar_rotation/sample019_targetPred.png} &
\includegraphics[height=\limfig cm]{figures/limitations/airplane_rot/sample009_source.png} &
\includegraphics[height=\limfig cm]{figures/limitations/airplane_rot/sample009_target.png} &
\includegraphics[height=\limfig cm]{figures/limitations/airplane_rot/sample009_targetPred.png} \\

source &
target &
warped &
source &
target & 
warped \\
 
\end{tabular}

%%%%%%%%%%%%%%%%%%

%\includegraphics[height=\limfig cm]{figures/limitations/airplanes_vase/sample001_source.png} &
%\includegraphics[height=\limfig cm]{figures/limitations/airplanes_vase/sample001_target.png} &
%\includegraphics[height=\limfig cm]{figures/limitations/airplanes_vase/sample001_targetPred.png} &
%\includegraphics[height=\limfig cm]{figures/limitations/airplanes_vase/sample001_targetPred_vase.png} \\
 
%source &
%target &
% &
% bottle \\

% \hline
% \addcomment{here}&
% \addcomment{goes}&
% \addcomment{failed}&
% \addcomment{rotation}\\

% Pears -> partial vases
	\jsubfig{\includegraphics[height=\limfig cm]{figures/limitations/airplanes_boat/sample027_source.png}} {}%
    \jsubfig{\includegraphics[height=\limfig cm]{figures/limitations/airplanes_boat/sample027_target.png}} {}%
    \jsubfig{\includegraphics[height=\limfig cm]{figures/limitations/airplanes_boat/sample027_targetPred.png}} {airplane}%
    \jsubfig{\includegraphics[height=\limfig cm]{figures/limitations/airplanes_boat/sample027_targetPred_vessel.png}} {vessel}%
    
    \jsubfig{\includegraphics[height=\limfig cm]{figures/limitations/airplanes_vase/sample001_source.png}} {}%
    \jsubfig{\includegraphics[height=\limfig cm]{figures/limitations/airplanes_vase/sample001_target.png}} {}%
    \jsubfig{\includegraphics[height=\limfig cm]{figures/limitations/airplanes_vase/sample001_targetPred.png}} {airplane}%
    \jsubfig{\includegraphics[height=\limfig cm]{figures/limitations/airplanes_vase/sample001_targetPred_vase.png}} {vase}%
\end{comment}

==> figures/limitations/topology.tex <==
\begin{figure}[h]
\newcommand{\limfig}{2}
\setlength\tabcolsep{5pt} % default value: 6pt
\begin{tabular}{c c c}

\includegraphics[height=\limfig cm]{figures/limitations/topology/sample155_source.png} &
\includegraphics[height=\limfig cm]{figures/limitations/topology/sample155_target.png} &
\includegraphics[height=\limfig cm]{figures/limitations/topology/sample155_targetPred.png} \\

%source &
%target &
% \\

\end{tabular}
\caption{\addcomment{Limitations of \ourmethod{} on different topologies.}}
\label{fig:limitations}
\end{figure}




\begin{comment}
/home/rana/dan3_local/localdata/silhouettes/rendered/multi_airplane/checkpoint/cagenet_2_12ctrls_silhouette,augmentAffine=t,batchSize=200,cage_reg=1e-05,classes=airplane,delCage=t,learn_beta=t,mpgPart=t/SatJan601:19:172018/qual
\end{comment}

==> figures/novel_class/figure.tex <==
\begin{figure}[h]

% violins -> partial guitars
% partial targets
	\jsubfig{}{}%
	\hfill \jsubfig{\includegraphics[height=1.6cm]{figures/novel_class/violins_guitars/sample003_target.png}} %{}%
    \hfill \jsubfig{\includegraphics[height=1.6cm]{figures/novel_class/violins_guitars/sample004_target.png}} %{}%
    \hfill \jsubfig{\includegraphics[height=1.6cm]{figures/novel_class/violins_guitars/sample027_target.png}} %{}%
    \hfill \jsubfig{\includegraphics[height=1.6cm]{figures/novel_class/violins_guitars/sample030_target.png}} {}%
    
% source1 & warps1
    \jsubfig{\includegraphics[height=1.6cm]{{figures/novel_class/violins_guitars/sample001_source.png}}} {}%
	\hfill \jsubfig{\includegraphics[height=1.6cm]{figures/novel_class/violins_guitars/sample003_targetPred.png}} %{}%
    \hfill \jsubfig{\includegraphics[height=1.6cm]{figures/novel_class/violins_guitars/sample004_targetPred.png}} %{}%
    \hfill \jsubfig{\includegraphics[height=1.6cm]{figures/novel_class/violins_guitars/sample027_targetPred.png}} %{}%
    \hfill \jsubfig{\includegraphics[height=1.6cm]{figures/novel_class/violins_guitars/sample030_targetPred.png}} {}%
\\
\jsubfig{\includegraphics[width=8cm]{{figures/novel_class/line.png}}} {}% 
\\
% kites -> partial airplanes    
% partial targets
	\jsubfig{}{}%
	\hfill \jsubfig{\includegraphics[height=1.6cm]{figures/novel_class/kites_airplanes/sample005_target.png}} %{}%
    \hfill \jsubfig{\includegraphics[height=1.6cm]{figures/novel_class/kites_airplanes/sample012_target.png}} %{}%
    \hfill \jsubfig{\includegraphics[height=1.6cm]{figures/novel_class/kites_airplanes/sample018_target.png}} %{}%
    \hfill \jsubfig{\includegraphics[height=1.6cm]{figures/novel_class/kites_airplanes/sample002_target.png}} {}%
    
% source1 & warps1
    \jsubfig{\includegraphics[height=1.6cm]{{figures/novel_class/kites_airplanes/sample001_source.png}}} {}%
	\hfill \jsubfig{\includegraphics[height=1.6cm]{figures/novel_class/kites_airplanes/sample005_targetPred.png}} %{}%
    \hfill \jsubfig{\includegraphics[height=1.6cm]{figures/novel_class/kites_airplanes/sample012_targetPred.png}} %{}%
    \hfill \jsubfig{\includegraphics[height=1.6cm]{figures/novel_class/kites_airplanes/sample018_targetPred.png}} %{}%
    \hfill \jsubfig{\includegraphics[height=1.6cm]{figures/novel_class/kites_airplanes/sample002_targetPred.png}} {}%
\\
\jsubfig{\includegraphics[width=8cm]{{figures/novel_class/line.png}}} {}% 
\\
% Lamps -> partial vases   
% partial targets
	\jsubfig{}{}%
	\hfill \jsubfig{\includegraphics[height=1.6cm]{figures/novel_class/lamps_vases/sample005_target.png}} %{}%
    \hfill \jsubfig{\includegraphics[height=1.6cm]{figures/novel_class/lamps_vases/sample006_target.png}} %{}%
    \hfill \jsubfig{\includegraphics[height=1.6cm]{figures/novel_class/lamps_vases/sample026_target.png}} %{}%
    \hfill \jsubfig{\includegraphics[height=1.6cm]{figures/novel_class/lamps_vases/sample029_target.png}} {}%
    
% source1 & warps1
    \jsubfig{\includegraphics[height=1.6cm]{{figures/novel_class/lamps_vases/sample001_source.png}}} {}%
	\hfill \jsubfig{\includegraphics[height=1.6cm]{figures/novel_class/lamps_vases/sample005_targetPred.png}} %{}%
    \hfill \jsubfig{\includegraphics[height=1.6cm]{figures/novel_class/lamps_vases/sample006_targetPred.png}} %{}%
    \hfill \jsubfig{\includegraphics[height=1.6cm]{figures/novel_class/lamps_vases/sample026_targetPred.png}} %{}%
    \hfill \jsubfig{\includegraphics[height=1.6cm]{figures/novel_class/lamps_vases/sample029_targetPred.png}} {}%

% Pears -> partial vases   
%	\jsubfig{{\hspace*{1.6 cm}}} {}  %
%	\hfill \jsubfig{\includegraphics[height=1.6cm]{figures/novel_class/pears_vases/sample003_target.png}} %{}%
%    \hfill \jsubfig{\includegraphics[height=1.6cm]{figures/novel_class/pears_vases/sample006_target.png}} %{}%
%    \hfill \jsubfig{\includegraphics[height=1.6cm]{figures/novel_class/pears_vases/sample008_target.png}} %{}%
%    \hfill \jsubfig{\includegraphics[height=1.6cm]{figures/novel_class/pears_vases/sample019_target.png}} {}%
    
% source1 & warps1
%    \jsubfig{\includegraphics[height=1.6cm]{{figures/novel_class/pears_vases/sample001_source.png}}} {}%
%	\hfill \jsubfig{\includegraphics[height=1.6cm]{figures/novel_class/pears_vases/sample003_targetPred.png}} %{}%
%    \hfill \jsubfig{\includegraphics[height=1.6cm]{figures/novel_class/pears_vases/sample006_targetPred.png}} %{}%
%    \hfill \jsubfig{\includegraphics[height=1.6cm]{figures/novel_class/pears_vases/sample008_targetPred.png}} %{}%
%    \hfill \jsubfig{\includegraphics[height=1.6cm]{figures/novel_class/pears_vases/sample019_targetPred.png}} {}%
\caption{Qualitative results on a novel class, unseen during training, that shares some semantic commonalities with the trained class. First pair of rows: \ourmethod{} trained on guitars, then evaluated on warping a violin to different partial guitars from the test set. Second pair of rows: \ourmethod{} trained on airplanes, then evaluated on warping a kite to different partial airplanes from the test set. \ourmethod{} trained on vases, then evaluated on warping a lamp to different partial vases from the test set.}
\label{fig:novel_classes}
\end{figure}

==> figures/novel_class_2/figure.tex <==
\begin{comment}
-data /home/rana/data/silhouettes/rendered/vase -retrain /home/rana/data/silhouettes/rendered/vase/checkpoint/cagenet_2_12ctrls_silhouette,augmentAffine=t,batchSize=200,cage_reg=1e-05,delCage=t,learn_beta=t,mpgPart=t,nEpochs=100/MonSep1119:22:422017/model_100.t7 -batchSize 30 -cage_reg 1e-5 -delCage -evalOnly -learn_beta -mpgPart -src_name ./../test_cache/texture_tests/pumpkin2.h5 -fullShapeflag

%squidward
-data /home/rana/data/silhouettes/rendered/guitar -retrain /home/rana/dan3/silhouettes/rendered/guitar/checkpoint/cagenet_2_12ctrls_silhouette,augmentAffine=t,batchSize=200,cage_reg=1e-05,delCage=t,learn_beta=t,nEpochs=100/MonSep421:20:022017/model_99.t7 -batchSize 30 -cage_reg 1e-5 -delCage -evalOnly -learn_beta -src_name ./../test_cache/texture_tests/ae1.h5 -mpgPart -mpgSRng 1.1..1.8 -mpgTRng -0.1..0.1


/home/rana/dan3/silhouettes/rendered/guitar/checkpoint/cagenet_2_12ctrls_silhouette,batchSize=50,cage_reg=1e-05,delCage=t,evalOnly=t,learn_beta=t,mpgPart=t,mpgSRng=1.1..1.8,mpgTRng=-0.1..0.1/SatSep1619:27:342017/qual
\end{comment}


\begin{figure*}[h]
	\newcommand{\nnfigb}{1.7}    
\setlength\tabcolsep{1pt} % default value: 6pt
\begin{tabular}{ c c c c c c c c c c}
% (rocket) targets
 & 
\includegraphics[width=\nnfigb cm]{figures/novel_class_2/rocket_airplanes/sample002_target.png} &
\includegraphics[width=\nnfigb cm]{figures/novel_class_2/rocket_airplanes/sample026_target.png} &
\includegraphics[width=\nnfigb cm]{figures/novel_class_2/rocket_airplanes/sample027_target.png} &
\includegraphics[width=\nnfigb cm]{figures/novel_class_2/rocket_airplanes/sample015_target.png} &
%  targets 
 & 
\includegraphics[width=\nnfigb cm]{figures/novel_class_2/bat3_airplanes/sample002_target.png} &
\includegraphics[width=\nnfigb cm]{figures/novel_class_2/bat3_airplanes/sample014_target.png} &
\includegraphics[width=\nnfigb cm]{figures/novel_class_2/bat3_airplanes/sample022_target.png} &
\includegraphics[width=\nnfigb cm]{figures/novel_class_2/bat3_airplanes/sample029_target.png} \\
%  rockets warped
\includegraphics[width=\nnfigb cm]{figures/novel_class_2/rocket_airplanes/sample001_source.png} &
\includegraphics[width=\nnfigb cm]{figures/novel_class_2/rocket_airplanes/sample002_targetPred.png} &
\includegraphics[width=\nnfigb cm]{figures/novel_class_2/rocket_airplanes/sample026_targetPred.png} &
\includegraphics[width=\nnfigb cm]{figures/novel_class_2/rocket_airplanes/sample027_targetPred.png} &
\includegraphics[width=\nnfigb cm]{figures/novel_class_2/rocket_airplanes/sample015_targetPred.png} &
%  bats warped
\includegraphics[width=\nnfigb cm]{figures/novel_class_2/bat3_airplanes/sample001_source.png} &
\includegraphics[width=\nnfigb cm]{figures/novel_class_2/bat3_airplanes/sample002_targetPred.png} &
\includegraphics[width=\nnfigb cm]{figures/novel_class_2/bat3_airplanes/sample014_targetPred.png} &
\includegraphics[width=\nnfigb cm]{figures/novel_class_2/bat3_airplanes/sample022_targetPred.png} &
\includegraphics[width=\nnfigb cm]{figures/novel_class_2/bat3_airplanes/sample029_targetPred.png} \\

% (jar) targets
 & 
\includegraphics[width=\nnfigb cm]{figures/novel_class/lamps_vases/sample005_target.png} &
\includegraphics[width=\nnfigb cm]{figures/novel_class/lamps_vases/sample006_target.png} &
\includegraphics[width=\nnfigb cm]{figures/novel_class/lamps_vases/sample026_target.png} &
\includegraphics[width=\nnfigb cm]{figures/novel_class/lamps_vases/sample029_target.png} &
%  (squidward) targets 
 & 
\includegraphics[width=\nnfigb cm]{figures/novel_class_2/squid_guitar/sample004_target.png} &
\includegraphics[width=\nnfigb cm]{figures/novel_class_2/squid_guitar/sample008_target.png} &
\includegraphics[width=\nnfigb cm]{figures/novel_class_2/squid_guitar/sample011_target.png} &
\includegraphics[width=\nnfigb cm]{figures/novel_class_2/squid_guitar/sample027_target.png} \\
%  jar warped
\includegraphics[width=\nnfigb cm]{figures/novel_class/lamps_vases/sample001_source.png} &
\includegraphics[width=\nnfigb cm]{figures/novel_class/lamps_vases/sample005_targetPred.png} &
\includegraphics[width=\nnfigb cm]{figures/novel_class/lamps_vases/sample006_targetPred.png} &
\includegraphics[width=\nnfigb cm]{figures/novel_class/lamps_vases/sample026_targetPred.png} &
\includegraphics[width=\nnfigb cm]{figures/novel_class/lamps_vases/sample029_targetPred.png} &
%  squidward warped
\includegraphics[width=\nnfigb cm]{figures/novel_class_2/squid_guitar/sample001_source.png} &
\includegraphics[width=\nnfigb cm]{figures/novel_class_2/squid_guitar/sample004_targetPred.png} &
\includegraphics[width=\nnfigb cm]{figures/novel_class_2/squid_guitar/sample008_targetPred.png} &
\includegraphics[width=\nnfigb cm]{figures/novel_class_2/squid_guitar/sample011_targetPred.png} &
\includegraphics[width=\nnfigb cm]{figures/novel_class_2/squid_guitar/sample027_targetPred.png} \\





\end{tabular}
\caption{Further results. Deforming a novel class source shape (unseen during training) that shares geometric commonalities with the trained class (test set).}
\label{fig:novel_classes_2}
\end{figure*}


\begin{comment}







% Lamps -> partial vases   
% partial targets
	\jsubfig{}{}%
	\hfill \jsubfig{\includegraphics[height=1.6cm]{figures/novel_class/lamps_vases/sample005_target.png}} %{}%
    \hfill \jsubfig{\includegraphics[height=1.6cm]{figures/novel_class/lamps_vases/sample006_target.png}} %{}%
    \hfill \jsubfig{\includegraphics[height=1.6cm]{figures/novel_class/lamps_vases/sample026_target.png}} %{}%
    \hfill \jsubfig{\includegraphics[height=1.6cm]{figures/novel_class/lamps_vases/sample029_target.png}} {}%
    
% source1 & warps1
    \jsubfig{\includegraphics[height=1.6cm]{{figures/novel_class/lamps_vases/sample001_source.png}}} {}%
	\hfill \jsubfig{\includegraphics[height=1.6cm]{figures/novel_class/lamps_vases/sample005_targetPred.png}} %{}%
    \hfill \jsubfig{\includegraphics[height=1.6cm]{figures/novel_class/lamps_vases/sample006_targetPred.png}} %{}%
    \hfill \jsubfig{\includegraphics[height=1.6cm]{figures/novel_class/lamps_vases/sample026_targetPred.png}} %{}%
    \hfill \jsubfig{\includegraphics[height=1.6cm]{figures/novel_class/lamps_vases/sample029_targetPred.png}} {}%

% rocket -> airplanes 
	\jsubfig{{\hspace*{\nnfigb cm}}} {}  %
	\hfill \jsubfig{\includegraphics[height=\nnfigb cm]{figures/novel_class_2/rocket_airplanes/sample002_target.png}} {}%
    \hfill \jsubfig{\includegraphics[height=\nnfigb cm]{figures/novel_class_2/rocket_airplanes/sample026_target.png}} {}%
    \hfill \jsubfig{\includegraphics[height=\nnfigb cm]{figures/novel_class_2/rocket_airplanes/sample027_target.png}} {}%
    \hfill \jsubfig{\includegraphics[height=\nnfigb cm]{figures/novel_class_2/rocket_airplanes/sample015_target.png}} {}%
    
% source1 & warps1
    \jsubfig{\includegraphics[height=\nnfigb cm]{{figures/novel_class_2/rocket_airplanes/sample001_source.png}}} {}%
	\hfill \jsubfig{\includegraphics[height=\nnfigb cm]{figures/novel_class_2/rocket_airplanes/sample002_targetPred.png}} {}%
    \hfill \jsubfig{\includegraphics[height=\nnfigb cm]{figures/novel_class_2/rocket_airplanes/sample026_targetPred.png}} {}%
    \hfill \jsubfig{\includegraphics[height=\nnfigb cm]{figures/novel_class_2/rocket_airplanes/sample027_targetPred.png}} {}%
    \hfill \jsubfig{\includegraphics[height=\nnfigb cm]{figures/novel_class_2/rocket_airplanes/sample015_targetPred.png}} {}%

	% bat -> airplanes     
    \jsubfig{{\hspace*{\nnfigb cm}}} {}  %
	\hfill \jsubfig{\includegraphics[height=\nnfigb cm]{figures/novel_class_2/bat3_airplanes/sample002_target.png}} {}%
    \hfill \jsubfig{\includegraphics[height=\nnfigb cm]{figures/novel_class_2/bat3_airplanes/sample014_target.png}} {}%
    \hfill \jsubfig{\includegraphics[height=\nnfigb cm]{figures/novel_class_2/bat3_airplanes/sample022_target.png}} {}%
    \hfill \jsubfig{\includegraphics[height=\nnfigb cm]{figures/novel_class_2/bat3_airplanes/sample029_target.png}} {}
    
    \jsubfig{\includegraphics[height=\nnfigb cm]{{figures/novel_class_2/bat3_airplanes/sample001_source.png}}} {}%
	\hfill \jsubfig{\includegraphics[height=\nnfigb cm]{figures/novel_class_2/bat3_airplanes/sample002_targetPred.png}} {}%
    \hfill \jsubfig{\includegraphics[height=\nnfigb cm]{figures/novel_class_2/bat3_airplanes/sample014_targetPred.png}} {}%
    \hfill \jsubfig{\includegraphics[height=\nnfigb cm]{figures/novel_class_2/bat3_airplanes/sample022_targetPred.png}} {}%
    \hfill \jsubfig{\includegraphics[height=\nnfigb cm]{figures/novel_class_2/bat3_airplanes/sample029_targetPred.png}} {}















% Pears -> partial vases   
	\jsubfig{{\hspace*{1.6 cm}}} {}  %
	\hfill \jsubfig{\includegraphics[height=\nnfigb cm]{figures/novel_class_2/pears_vases/sample003_target.png}} {}%
    \hfill \jsubfig{\includegraphics[height=\nnfigb cm]{figures/novel_class_2/pears_vases/sample006_target.png}} {}%
    \hfill \jsubfig{\includegraphics[height=\nnfigb cm]{figures/novel_class_2/pears_vases/sample008_target.png}} {}%
    \hfill \jsubfig{\includegraphics[height=\nnfigb cm]{figures/novel_class_2/pears_vases/sample019_target.png}} {}%
    
% source1 & warps1
    \jsubfig{\includegraphics[height=\nnfigb cm]{{figures/novel_class_2/pears_vases/sample001_source.png}}} {}%
	\hfill \jsubfig{\includegraphics[height=\nnfigb cm]{figures/novel_class_2/pears_vases/sample003_targetPred.png}} {}%
    \hfill \jsubfig{\includegraphics[height=\nnfigb cm]{figures/novel_class_2/pears_vases/sample006_targetPred.png}} {}%
    \hfill \jsubfig{\includegraphics[height=\nnfigb cm]{figures/novel_class_2/pears_vases/sample008_targetPred.png}} {}%
    \hfill \jsubfig{\includegraphics[height=\nnfigb cm]{figures/novel_class_2/pears_vases/sample019_targetPred.png}} {}%
    
% Pumpkins -> partial vases   
	\jsubfig{{\hspace*{\nnfigb cm}}} {}  %
	\hfill \jsubfig{\includegraphics[height=\nnfigb cm]{figures/novel_class_2/pumpkin_vases/sample002_target.png}} {}%
    \hfill \jsubfig{\includegraphics[height=\nnfigb cm]{figures/novel_class_2/pumpkin_vases/sample004_target.png}} {}%
    \hfill \jsubfig{\includegraphics[height=\nnfigb cm]{figures/novel_class_2/pumpkin_vases/sample011_target.png}} {}%
    \hfill \jsubfig{\includegraphics[height=\nnfigb cm]{figures/novel_class_2/pumpkin_vases/sample012_target.png}} {}%
    
% source1 & warps1
    \jsubfig{\includegraphics[height=\nnfigb cm]{{figures/novel_class_2/pumpkin_vases/sample001_source.png}}} {}%
	\hfill \jsubfig{\includegraphics[height=\nnfigb cm]{figures/novel_class_2/pumpkin_vases/sample002_targetPred.png}} {}%
    \hfill \jsubfig{\includegraphics[height=\nnfigb cm]{figures/novel_class_2/pumpkin_vases/sample004_targetPred.png}} {}%
    \hfill \jsubfig{\includegraphics[height=\nnfigb cm]{figures/novel_class_2/pumpkin_vases/sample011_targetPred.png}} {}%
    \hfill \jsubfig{\includegraphics[height=\nnfigb cm]{figures/novel_class_2/pumpkin_vases/sample012_targetPred.png}} {}%
\\
\jsubfig{\includegraphics[width=8cm]{{figures/novel_class/line.png}}} {}% 
\\
% Squid -> guitars 
	\jsubfig{{\hspace*{\nnfigb cm}}} {}  %
	\hfill \jsubfig{\includegraphics[height=\nnfigb cm]{figures/novel_class_2/squid_guitar/sample004_target.png}} {}%
    \hfill \jsubfig{\includegraphics[height=\nnfigb cm]{figures/novel_class_2/squid_guitar/sample008_target.png}} {}%
    \hfill \jsubfig{\includegraphics[height=\nnfigb cm]{figures/novel_class_2/squid_guitar/sample011_target.png}} {}%
    \hfill \jsubfig{\includegraphics[height=\nnfigb cm]{figures/novel_class_2/squid_guitar/sample027_target.png}} {}%
    
% source1 & warps1
    \jsubfig{\includegraphics[height=\nnfigb cm]{{figures/novel_class_2/squid_guitar/sample001_source.png}}} {}%
	\hfill \jsubfig{\includegraphics[height=\nnfigb cm]{figures/novel_class_2/squid_guitar/sample004_targetPred.png}} {}%
    \hfill \jsubfig{\includegraphics[height=\nnfigb cm]{figures/novel_class_2/squid_guitar/sample008_targetPred.png}} {}%
    \hfill \jsubfig{\includegraphics[height=\nnfigb cm]{figures/novel_class_2/squid_guitar/sample011_targetPred.png}} {}%
    \hfill \jsubfig{\includegraphics[height=\nnfigb cm]{figures/novel_class_2/squid_guitar/sample027_targetPred.png}} {}%
    \\
	\jsubfig{\includegraphics[width=8cm]{{figures/novel_class/line.png}}} {}% 
	\\

% bat -> airplanes     
    \jsubfig{{\hspace*{\nnfigb cm}}} {}  %
	\hfill \jsubfig{\includegraphics[height=\nnfigb cm]{figures/novel_class_2/bat_airplanes/sample012_target.png}} {}%
    \hfill \jsubfig{\includegraphics[height=\nnfigb cm]{figures/novel_class_2/bat_airplanes/sample022_target.png}} {}%
    \hfill \jsubfig{\includegraphics[height=\nnfigb cm]{figures/novel_class_2/bat_airplanes/sample027_target.png}} {}%
    \hfill \jsubfig{\includegraphics[height=\nnfigb cm]{figures/novel_class_2/bat_airplanes/sample029_target.png}} {}
    
    \jsubfig{\includegraphics[height=\nnfigb cm]{{figures/novel_class_2/bat_airplanes/sample001_source.png}}} {}%
	\hfill \jsubfig{\includegraphics[height=\nnfigb cm]{figures/novel_class_2/bat_airplanes/sample012_targetPred.png}} {}%
    \hfill \jsubfig{\includegraphics[height=\nnfigb cm]{figures/novel_class_2/bat_airplanes/sample022_targetPred.png}} {}%
    \hfill \jsubfig{\includegraphics[height=\nnfigb cm]{figures/novel_class_2/bat_airplanes/sample027_targetPred.png}} {}%
    \hfill \jsubfig{\includegraphics[height=\nnfigb cm]{figures/novel_class_2/bat_airplanes/sample029_targetPred.png}} {}
\end{comment}

==> figures/rot/figure.tex <==
\begin{figure}
\newcommand{\rotfig}{1.9}
\setlength\tabcolsep{3pt}
\begin{tabular}{c c c c}


\includegraphics[width=\rotfig cm]{figures/rot/airplanes_r/sample141_source.png} &
\includegraphics[width=\rotfig cm]{figures/rot/airplanes_r/sample141_target.png} &
\includegraphics[width=\rotfig cm]{figures/rot/airplanes_str/sample141_targetPred.png} &
\includegraphics[width=\rotfig cm]{figures/rot/airplanes_r/sample141_targetPred.png} \\

%\hline

%\includegraphics[width=\rotfig cm]{figures/rot/airplanes_r/sample343_source.png} &
%\includegraphics[width=\rotfig cm]{figures/rot/airplanes_r/sample343_target.png} &
%\includegraphics[width=\rotfig cm]{figures/rot/airplanes_str/sample343_targetPred.png} &
%\includegraphics[width=\rotfig cm]{figures/rot/airplanes_r/sample343_targetPred.png} \\

source  &
target  &
baseline  &
augmented  \\


\end{tabular}
\caption{Robustness to orientation deviations. 
We align a source shape to a target with a deviated orientation. Results in the third column are obtained with \ourmethod{} trained on the original airplane dataset and show inability to recover target orientation. Conversely, results in the fourth column are obtained with \ourmethod{} trained on the same set with added augmentation of orientation perturbations of up to $\pm 15^{\circ}$, and demonstrate correct orientation recovery and the potential to handle heterogeneously oriented datasets or imperfect orientation pre-processing.}
%Training on the airplane dataset augmented with orientation perturbations of up to $\pm 15^{\circ}$. Qualitative examples demonstrate FFDnet ability to handle imperfections in the pre-processed orientation.}}
\label{fig:rots}
\end{figure}




















\begin{comment}

%\includegraphics[width=\rotfig cm]{figures/rot/airplanes_str_str/sample141_source.png}  & 
%\includegraphics[width=\rotfig cm]{figures/rot/airplanes_str_str/sample141_target.png} &
%\includegraphics[width=\rotfig cm]{figures/rot/airplanes_str_str/sample141_targetPred.png} \\

%\includegraphics[width=\rotfig cm]{figures/rot/airplanes_r/sample343_source.png}  & 
%\includegraphics[width=\rotfig cm]{figures/rot/airplanes_str_str/sample343_target.png} &
%\includegraphics[width=\rotfig cm]{figures/rot/airplanes_str_str/sample343_targetPred.png} \\


%\hline
%\includegraphics[width=\rotfig cm]{figures/rot/airplanes_str_str/sample744_source.png}  & 
%\includegraphics[width=\rotfig cm]{figures/rot/airplanes_str_str/sample744_target.png} &
%\includegraphics[width=\rotfig cm]{figures/rot/airplanes_str_str/sample744_targetPred.png} \\
% &
%\includegraphics[width=\rotfig cm]{figures/rot/airplanes_r/sample744_target.png} &
%\includegraphics[width=\rotfig cm]{figures/rot/airplanes_r/sample744_targetPred.png} \\

\includegraphics[width=\rotfig cm]{figures/rot/airplanes_str_str/sample331_source.png}  & 
\includegraphics[width=\rotfig cm]{figures/rot/airplanes_str_str/sample331_target.png} &
\includegraphics[width=\rotfig cm]{figures/rot/airplanes_str_str/sample331_targetPred.png} \\

\includegraphics[width=\rotfig cm]{figures/rot/airplanes_r/sample331_source.png}  & 
\includegraphics[width=\rotfig cm]{figures/rot/airplanes_r/sample331_target.png} &
\includegraphics[width=\rotfig cm]{figures/rot/airplanes_r/sample331_targetPred.png} \\



343 // 341





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%% STRAIGHT TRAIN / TEST %%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
th main.lua -data /home/rana/data/silhouettes/rendered/airplane -retrain /home/rana/data/silhouettes/rendered/airplane/checkpoint/cagenet_2_12ctrls_silhouette,batchSize=200,cage_reg=1e-05,delCage=t,learn_beta=t/ThuJul2701:53:192017/model_49.t7 -cage_reg 1e-5 -delCage -evalOnly -learn_beta

/home/rana/data/silhouettes/rendered/airplane/checkpoint/cagenet_2_12ctrls_silhouette,cage_reg=1e-05,delCage=t,evalOnly=t,learn_beta=t/TueSep1917:11:452017/qual

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%% ROT TRAIN / TEST %%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
th main.lua -data /home/rana/data/silhouettes/rendered/airplane -retrain /home/rana/data/silhouettes/rendered/airplane/checkpoint/cagenet_2_12ctrls_silhouette,RRng=-0.25..0.25,augmentAffine=t,batchSize=200,cage_reg=1e-05,delCage=t,learn_beta=t,nEpochs=150/SunSep1718:50:012017/model_100.t7 -cage_reg 1e-5 -delCage -evalOnly -learn_beta -RRng -0.2..-0.2 -mpgRRng -0.2..-0.2

/home/rana/data/silhouettes/rendered/airplane/checkpoint/cagenet_2_12ctrls_silhouette,RRng=-0.2..-0.2,cage_reg=1e-05,delCage=t,evalOnly=t,learn_beta=t,mpgRRng=-0.2..-0.2/TueSep1917:48:432017/qual


\includegraphics[width=\nnfig cm]{figures/novel_novel_class/bat1bat2/sample002_source.png} 


th main.lua -data /home/rana/data/silhouettes/rendered/airplane -retrain /home/rana/data/silhouettes/rendered/airplane/checkpoint/cagenet_2_12ctrls_silhouette,RRng=-0.25..0.25,augmentAffine=t,batchSize=200,cage_reg=1e-05,delCage=t,learn_beta=t,nEpochs=150/SunSep1718:50:012017/model_100.t7 -evalOnly -batchSize 30 -cage_reg 1e-05 -delCage -learn_beta

/home/rana/data/silhouettes/rendered/airplane/checkpoint/cagenet_2_12ctrls_silhouette,batchSize=30,cage_reg=1e-05,delCage=t,evalOnly=t,learn_beta=t/TueSep1909:22:102017/qual



%rotated
/home/rana/data/silhouettes/rendered/airplane/checkpoint/cagenet_2_12ctrls_silhouette,RRng=-0.25..-0.25,batchSize=30,cage_reg=1e-05,delCage=t,evalOnly=t,learn_beta=t/TueSep1909:51:012017/qual

%straight
/home/rana/data/silhouettes/rendered/airplane/checkpoint/cagenet_2_12ctrls_silhouette,batchSize=30,cage_reg=1e-05,delCage=t,evalOnly=t,learn_beta=t/TueSep1909:22:102017/qual

\end{comment}

==> figures/threeD/seg/figure2.tex <==
\begin{figure}[h!]
\newcommand{\tfig}{2.7}
\newcommand{\vfig}{1.7}
\setlength\tabcolsep{10pt}
\begin{tabular}{c c}

%vase
\adjincludegraphics[width=\vfig cm,trim={{.3\width} {.18\height} {.3\width} {.15\height}},clip]{figures/threeD/seg/vase/0036.png} &
\adjincludegraphics[width=\vfig cm,trim={{.3\width} {.18\height} {.3\width} {.15\height}},clip]{figures/threeD/seg/vase/0036_0196.png} \\

\adjincludegraphics[width=\vfig cm,trim={{.3\width} {.15\height} {.3\width} {.1\height}},clip]{figures/threeD/seg/vase/0097.png} &
\adjincludegraphics[width=\vfig cm,trim={{.3\width} {.15\height} {.3\width} {.1\height}},clip]{figures/threeD/seg/vase/0097_0158.png} \\

\adjincludegraphics[width=\vfig cm,trim={{.25\width} {.15\height} {.2\width} {.15\height}},clip]{figures/threeD/seg/vase/0014.png} &
\adjincludegraphics[width=\vfig cm,trim={{.25\width} {.15\height} {.2\width} {.15\height}},clip]{figures/threeD/seg/vase/0014_0054.png} \\

%airplane
\adjincludegraphics[width=\tfig cm,trim={{.3\width} {.35\height} {.25\width} {.33\height}},clip]{figures/threeD/seg/airplane/601.png} &
\adjincludegraphics[width=\tfig cm,trim={{.3\width} {.35\height} {.25\width} {.33\height}},clip]{figures/threeD/seg/airplane/601_602.png} \\

\adjincludegraphics[width=\tfig cm,trim={{.3\width} {.3\height} {.25\width} {.3\height}},clip]{figures/threeD/seg/airplane/005.png} &
\adjincludegraphics[width=\tfig cm,trim={{.28\width} {.3\height} {.2\width} {.25\height}},clip]{figures/threeD/seg/airplane/005_007.png} \\

\adjincludegraphics[width=\tfig cm,trim={{.3\width} {.3\height} {.25\width} {.3\height}},clip]{figures/threeD/seg/airplane/006.png} &
\adjincludegraphics[width=\tfig cm,trim={{.3\width} {.3\height} {.25\width} {.3\height}},clip]{figures/threeD/seg/airplane/006_1949.png} \\

segmented &
transferred \\

\end{tabular}    
\caption{\ourmethod{} results on 3D segmentation transfer (test set). The labels in the source shape (left) transfered to the target shapes using \ourmethod{} (right). The estimated alignment is used in combination with a simple graph cut optimization as a post process.} 
\label{fig:threeD_seg}
\end{figure}


%. Using only graph cut optimization without alignment is shown in the center column (naive).

==> figures/threeD/texture/figure.tex <==
\begin{figure}
\newcommand{\tfig}{3}
\setlength\tabcolsep{1pt}
\begin{tabular}{c c c}


\includegraphics[width=\tfig cm]{figures/threeD/texture/orig.png} &
\includegraphics[width=\tfig cm]{figures/limitations/temp.png} &
\includegraphics[width=\tfig cm]{figures/threeD/texture/warped_0036c.png} \\

source &
target &
deformed \\

\end{tabular}    
\caption{\addcomment{Using \ourmethod{} to deform a 3D model containing hand-crafted render parameters.}}
\label{fig:threeD_txt}
\end{figure}

==> method_old.tex <==
\section{Methodology}

\subsection{FFD Computation via Unsupervised Learning}

%% orig
The input to our system is made up of pairs of source and target shapes, where a target shape may be partial at various locations and to varying extents. The baseline system consists of a neural network component $f$ that computes a FFD in the form of a low resolution grid-based warp field $W_c$, followed by a bilinear upsampling component that produces the full resolution warp to be applied on the source shape. Since the ground-truth FFD which correctly aligns the source to the target shape is unknown, our unsupervised scheme facilitates training by bestowing a self-supervised loss function: comparing the warped source to the full target (see Figure~\ref{fig:FFD_arch}). 
%thus, for self-supervision, the loss function compares the warped source to the full target (see Figure~\ref{fig:FFD_arch}).

The input source shape $S$ and the potentially partial target $T^p$ are stacked as a two channel image and passed to $f$ to obtain the low resolution FFD warp field: $f(S,T^p) = W_c$. The architecture of $f$ is given by a series of max pooling, convolutions and rectified linear activation units (repeated four times), followed by two linear layers. Similar to~\cite{spatialtransformer}, we train the network from scratch: setting the convolutional layer weights randomly, and initializing the linear component to yield the identity displacement field (weights set to zero and biases to the identity displacement field).

\begin{figure}[h]
\jsubfig{\includegraphics[height=3cm]{figures/FFD/source.png}} {}%
\; \jsubfig{\includegraphics[height=3cm]{figures/FFD/warped.png}} {}%
\\
\jsubfig{Source} {}%
\hspace*{2cm}
\jsubfig{Target} {}%
\caption{FFD illustration. The uniform 8x8 grid in the target domain shown in blue, applied in a backwards manner: each location in the target grid corresponds to a look-up location in the source.}
\label{fig:FFD_visualization}
\end{figure}

The displacement map used to express the FFD is a 2-dimensional displacement field, of smaller resolution than the source shape. Warping the source shape with the lower resolution grid is done through a 2-step bilinear sampling operation. First, use the bilinear sampler $\oland$ to upsample the lower resolution grid $W_c$ to the full size of the source image ($mxn$) by $W = W_c \oland \mathcal{G}^{mxn}$,
%\begin{equation}
%W = W_c \oland \mathcal{G}^{mxn},
%\label{eq:upsamplewc}
%\end{equation}
where $\mathcal{G}^{mxn}$ is a regular grid of coordinates for every pixel in the full resolution $mxn$. 
The second sampling applies the upsampled warp field on the source shape $\hat{T} = S \oland W$,
%\begin{equation}
%\hat{T} = S \oland W,
%\label{eq:lookupS}
%\end{equation}
resulting in an estimate of the target shape. For brevity, we represent the two-step sampling as
\begin{equation}
\hat{T} = S \oland W_c \leftarrow S \oland  (W_c \oland \mathcal{G}^{mxn}).
\label{eq:sampler}
\end{equation}

\begin{comment}
%The self-supervision layers warp the input source shape by the estimated FFD via a two-step backwards bilinear interpolation. 
The displacement map used to define the FFD is defined on a uniformly spaced grid, $\mathcal{G}^{w_c}_i = (x^{w_c}_i, y^{w_c}_i)$ of 2-dimensional displacements that is of smaller resolution than the source shape. Similarly, the source image intensities are defined on a uniformly spaced grid $\mathcal{G}$ of pixel locations $\mathcal{G}^s_i = (x^s_i, y^s_i)$, with normalized coordinates such that $-1 \leq x^s_i, y^s_i \leq 1$ lies within the confines of the source image. 

Applying the FFD $W_c$ on the source image ($S$) requires first upsampling the lower dimensional FFD to the full size of the image, $\mathcal{G}^w = \mathcal{G}^{w_c} \oland \mathcal{G}^s$, where $\oland$ represents backwards bilinear interpolation. Each pixel location in the regular target grid (Figure~\ref{fig:FFD_visualization} right) and the corresponding displacement vector which points to a location in the source (Figure~\ref{fig:FFD_visualization} left) are used to warp the source. The warped source image that is aligned to the target is given by $\hat{T} = S \oland \mathcal{G}^w$. For brevity, we represent the two-step mapping as ${\hat{T} = S \oland \mathcal{G}^{w_c} \leftarrow S \oland  (\mathcal{G}^{w_c} \oland \mathcal{G}^s)}$. See Figure~\ref{fig:FFD_visualization} for a visualization of an 8x8 FFD.
\end{comment}
%
The self-supervised training loss evaluates the difference between the complete target $T$ and the source that has been aligned by the FFD (\emph{i.e.,} estimated target $\hat{T}$) to train FFDnet. For every source $S^n$ and target $T^n$ example in the training set ($\mathcal{N}$), we train the network by minimizing the loss given by
%
\begin{equation}
%\begin{split}
f = \argmin_{f} 
\sum_{n \in \forall \mathcal{N}}
|| S^{n} \oland f(S^{n},{T^{p}}^n) - T^{n} || 
= \sum_{n \in \forall \mathcal{N}}
|| S^{n} \oland W_c - T^{n} ||,
%\\ 
%& = \sum_{\substack{S^{n} \in \forall S\\
%				T^{n} \in \forall T}} || S^{n} \oland W_c - T^{n} ||,
%\end{split}
\label{eq:FFDnet_loss}
\end{equation}
where $||\cdot||$ can be any error measure ({\em e.g.,} $\ell_1$-norm or $\ell_2$-norm). We use the smooth Huber loss, which is more robust to outliers than $\ell_2$-norm and more accurate on inliners compared to the $\ell_1$-norm. The Huber loss, computed for every pixel $i$ in the target and estimated target, is given by 
%
\begin{equation}
 L^H(T,\hat{T}) = \sum_{i \in \forall (\hat{T},T)} \left\{
                \begin{array}{ll}
                  \frac{1}{2}(T_i-\hat{T_i})^2 \quad \quad \textrm{for} \: |T_i-\hat{T_i}|< 1, \\
                  |T_i-\hat{T_i}| - \frac{1}{2} \quad \: \textrm{otherwise.}
                \end{array}
              \right.
\label{eq:huber}
\end{equation}

The proposed approach enables training without ground-truth FFDs while simultaneously learning to be partial-shape agnostic. At test time, given a source shape $S$ and a target shape with different parts missing $T^{p_1}, T^{p_2}, \cdots T^{p_n} \in T$ (from test set), FFDnet demonstrates partiality-agnostic behavior by computing very similar FFDs for different partialities of the same underlying target (see Figure~\ref{fig:sweeping_partialT}). We attribute this generalization to the unsupervised nature of the training process.

%Note that if the shapes are full (non-partial) we can optimize for the analytical upper bound (described in Appendix~\ref{sec:optimization}).
\subsection{FFD Regularization}
%Estimating the FFD without direct supervision, warrants FFDnet to falsely conjecture about the possible deformation field. Solely relying on the self-supervised paradigm defined in Equation~\ref{eq:FFDnet_loss} is ill-posed, since the large degree of freedom in FFDs may yield wildly different deformations, all with very similar cost.
Estimating FFDs without direct supervision, as in Equation~\ref{eq:FFDnet_loss}, is ill-posed, since the large degree of freedom in the FFD results in wildly different deformations all with very similar cost. Specifically, FFDnet operates solely on binary silhouettes, since knowing the true corresponding RGB textures between source and target shapes requires a form of ground-truth annotation. Binary silhouettes are problematic since any FFD which deforms source foreground pixels to target foreground pixels, even if parts are completely rearranged, results in the same loss. Absent regularization, FFDnet is entitled to falsely conjecture about the possible deformation field. Therefore, we incorporate two different types of regularization, enforcing axial monotonicity and encouraging piecewise smooth deformation fields (illustrated in Figure~\ref{fig:FFD_regularization}). As explained below, implementing these modifications becomes straight-forward when representing the FFD as a \emph{differential} displacement grid. 

\begin{figure}[h!]
\includegraphics[height=5cm]{figures/cagenet/FFD_regularization.png}
\caption{Supplementary regularization component commissioned for training FFDnet to compute favorable FFD grids. The network weights predict a differential grid which is first passed through absolute value operator to enforce axial monotonicity. Followed by anisotropic total variation identity regularization, encouraging piecewise-smooth deformation fields. Lastly, the $\cumsum$ layer restores the absolute displacement grid.}
\label{fig:FFD_regularization}
\end{figure}

\subsubsection{Differential Displacement Grids}
%nstead of directly estimating the FFD displacement field, we propose to estimate a displacement field that is relative to the preceding value in the grid, which, when summed cumulatively, results in the absolute displacement field.
We propose estimating a differential displacement grid, where each value is relative to the preceding value in the grid. Instead of directly computing the absolute FFD values from the CNN weights, we use the CNN weights to compute the differential FFD values which when cumulatively summed result in a absolute FFD grid. The differential displacement grid has desirable properties to facilitate favorable FFD computation (\emph{e.g.,} enforcing axial monotonicity and anisotropic total variation identity regularization). Furthermore, since we are using shared convolutional weights the smaller dynamic range gives the network higher precision (similarly observed in other deep learning approaches, such as super-resolution~\cite{kim2016accurate}). 

To illustrate differential displacement fields, consider a $1$-dimensional absolute sequence $a$ of length n, and the corresponding differential sequence $\Delta a$ as
\begin{subequations}
\begin{align}
a  & = \Big\{ a_k \Big\}_{k=1}^n  = ( a_1, a_2, a_3, \cdots, a_n ) \label{eq:oned_seq_abs}\\
\begin{split}
\Delta a & = \Big\{a_k - a_{k-1} \Big\}_{k=1}^n = ( \Delta a_1, \Delta a_2, \Delta a_3, \cdots, \Delta a_n )
\\
& = (a_1 - a_0, a_2 - a_1, a_3 - a_2,  \cdots, a_n - a_{n-1} ),
\end{split}
\label{eq:oned_seq_rel}
%\Delta a & = \left(a_k - a_{k-1} \right)_{k=1}^n  = (a_1 - a_0, a_2 - a_1, a_3 - a_2,  \cdots, a_n - a_{n-1} ) \label{eq:oned_seq_rel}
\end{align}
\end{subequations}
where $a_0$ is a scalar offset (here $a_0 = 0$). Given the differential $1$d-sequence $\Delta a$, the absolute sequence can be exactly recovered using the cumulative sum operator
\begin{equation}
a = \cumsum( \Delta a ,a_0) = \Big\{ \sum_{i=1}^k \Delta a_i \Big\}_{k=1}^n
\label{eq:cumsum}
\end{equation}
The proposed $\cumsum$ layer is differentiable and can be added into a network for training, it is easy to see in the $1$d-example that the derivative is given by
\begin{equation}
\partial \Delta a = \Big\{ \sum_{i}^k \partial  \Delta a_i \Big\}_{k=1}^n
\label{eq:cumsum_deriv}
\end{equation}
%

The deformation field in FFDnet is a $2$d grid with vertical and horizontal displacement components, where the $\cumsum$ operates along each dimension, respectively. The learned FFDnet weights map the input shapes to the differential displacement field $\Delta W_c$, subsequently passing through the $\cumsum$-layer, resulting in the final displacement field $W_c = \cumsum(\Delta W_c, W_0)$ (where $W_0$ is a learned scalar).

\subsubsection{Axial Monotonicity}
Observe that for any strictly positive differential $1$d-sequence ($\Delta a_k > 0$ for all $k$), the recovered absolute $1$d-sequence sequence $a$ is strictly monotonic
\begin{equation}
k \longmapsto a_k \because a \triangleq \cumsum(\Delta a, a_0) \textrm{ , where } \Delta a_k > 0 \textrm{ for all } k.
\label{eq:cumsum_mono}
\end{equation}
%
In FFDnet, we map the differential sequence at the end of the network to any positive codomain, for example by employing the absolute value operator. In the $2$d case, enforcing strictly positive relative displacement values $\Delta W_c > 0$, we ensure axial monotonicity in the displacement fields. Axial monotonicity means that each axis is monotonically increasing independently of the opposing axis.

\subsubsection{Anisotropic Total Variation Identity Regularization}
The differential displacement formulation yields interesting properties for encouraging piecewise smooth deformation fields in the form of TV regularization. Observe that the differential sequence as defined in Equation~\ref{eq:oned_seq_rel}, is actually the gradient of the absolute sequence in Equation~\ref{eq:oned_seq_abs}. 
Similarly for the $2$d counterpart, differential grid $\Delta W$ is made up of two channels, $\Delta W_x$,$\Delta W_y$, which are the horizontal and vertical derivatives of $W$ respectively. Recall that the anisotropic total variation regularization for a $2$d matrix is given by the $\ell_1$-norm of the sum of the horizontal and vertical gradients
%
\begin{equation}
V_{ani}(W) = ||\Delta Wx ||_1 + ||\Delta Wy ||_1.
\label{eq:TV_reg}
\end{equation}
%
TV regularization encourages deformations that are piecewise smooth: favoring smoothness but simultaneously allowing for large discontinuities due to the $\ell_1$-norm. Piecewise smoothness is the essence of a favorable deformation field: large discontinuities at the shape boundaries with a smooth shape interior. 

However, the lowest cost displacement field $W$ in the standard TV regularization from Equation~\ref{eq:TV_reg} would be a zero valued differential displacement field, an undesirable result. Instead, we encourage a non-zero-valued uniform spacing by subtracting the differential identity warp field from the differential warp: favoring a uniformly spaced grid over the size of the image.

%
For a $1$d analogy, consider an identity sequence $I$ of length $n$ normalized to the interval $[-1, 1]$, which is uniformly spaced by a scalar $\delta_n = \frac{2}{n-1} $. Then we can write $I$ and the corresponding differential $\Delta I$ as
%
\begin{subequations}
\begin{align}
\begin{split}
\label{eq:id_seq}
I & = \Big\{ -1 + (k - 1) \cdot \delta_n  \Big\}_{k=1}^n \\ 
& = (-1, -1 +\delta_n  , -1 +2 \delta_n , \cdots, 1)
\end{split}
\\
\label{eq:id_seq_rel}
\Delta I & = \Big\{ \delta_n  \Big\}_{k=1}^n
\end{align}
\end{subequations}
%
Where the differential identity sequence $\Delta I$ contains a single unique value: the uniform spacing constant $\delta_n$. In $2$d it follows that the proposed anisotropic TV identity regularization becomes 
%
\begin{equation}
V_{I} = V_{ani}(W - I) = ||\Delta Wx - \Delta Ix||_1 + ||\Delta Wy  - \Delta Iy||_1.
\label{eq:TV_reg_id}
\end{equation}
%
The overall contribution of the regularization term is controlled by a weighting factor $\lambda V_{I}$.

\begin{comment}
The differential displacement formulation yields interesting properties for encouraging smoothness, specifically in the form of encouraging piecewise smooth deformation fields. Note that the absolute identity FFD (non-relative) is given by uniformly spaced grid between $[-1, 1]$. Meaning, $W^I_c$ defined on a $mxm$ sized grid, sweeps in increments of $\delta_m = \frac{2}{m-1}$ such that $[-1, -1 +\delta_m, -1 + 2\cdot \delta_m, \cdots, 1]$ in both dimensions. However, the relative FFD identity $\Delta W^I_c$ simply contains a single scalar ($\delta_m$) for all entries of the grid $\Delta W^I_c \triangleq \frac{2}{m-1}$. Therefore, we incorporate an additional cost for deviating from the identity deformation in the form of
%
\begin{equation}
\lambda \cdot ||\Delta W_c - \delta_m||_1,
\label{eq:id_ffd}
\end{equation}
where $\lambda$ is the parameter used to regulate smoothness, and $||\cdot||_1$ is the $\ell_1$-norm. 
%#TODO: Change all paper to be consistent with either \ell or \mathcal{L}
\end{comment}



\begin{comment}
The input shapes are fed-forward through a series of neural network layers $f$, which map them to a FFD ($W_c$). Specifically, the input source shape $S$ and the (potentially partial) target $T^p$ are stacked as a two channel image $f(S,T^p) = W_c$. The architecture of $f$ is given by a series of max pooling, convolutions and rectified linear activation units (series repeated four times). Followed by two linear layers (regression parameterized by multiplicative weights and additive biases). We train from scratch setting the convolutional layer weights randomly, and initializing the linear layer to yield the identity displacement field (weights zero and biases identity field).

\begin{figure}[h]
\jsubfig{\includegraphics[height=3cm]{figures/FFD/source.png}} {}%
\; \jsubfig{\includegraphics[height=3cm]{figures/FFD/warped.png}} {}%
\caption{FFD illustration. The uniform 8x8 grid in the target domain shown in blue (right), applied in a backwards manner from the target to the source (right).}
\label{fig:FFD_visualization}
\end{figure}

The ground-truth FFD which correctly aligns the source to the target shape is unknown during training, so we proceed to feed-forward the resulting FFD through the self-supervision layers to enable an alternative training loss. The self-supervision layers warp the input source shape by the estimated FFD via a two-step backwards bilinear interpolation. The FFD displacements are defined on a uniformly spaced grid, $\mathcal{G}^{w_c}_i = (x^{w_c}_i, y^{w_c}_i)$ of 2-dimensional displacements that is of smaller resolution than the source shape. Similarly, the source image intensities are defined on a uniformly spaced grid $\mathcal{G}$ of pixel locations $\mathcal{G}^s_i = (x^s_i, y^s_i)$, with normalized coordinates such that $-1 \leq x^s_i, y^s_i \leq 1$ lies within the confines of the source image. Applying the FFD on the source image ($S$) requires first upsampling the lower dimensional FFD to the full size of the image, $\mathcal{G}^w = \mathcal{G}^{w_c} \oland \mathcal{G}^s$, where $\oland$ represents backwards bilinear interpolation. Then the full displacement field is used to warp the source image, to align it with the target $\hat{T} = S \oland \mathcal{G}^w$. For brevity, we represent the two step sampling as ${\hat{T} = S \oland \mathcal{G}^{w_c} \leftarrow S \oland  (\mathcal{G}^{w_c} \oland \mathcal{G}^s)}$ See Figure~\ref{fig:FFD_visualization} for a visualization of an 8x8 FFD.

The self-supervised training loss evaluates the difference between the complete target $T$ and the source warped by the FFD (estimated target $\hat{T}$) to train FFDnet. For every source and target example in the training set $(S_i, T_i)$, we train the network by minimizing the loss given by

\begin{equation}
%f = \min_{f} \sum_{S_i \in S, (T^p_i, T_i) \in T} || S \oland f(S_i,T^p_i) - T_i || = || S_i \oland W_c - T_i ||
f = \min_{f} 
\sum_{\substack{S_i \in \forall S\\
				T_i \in \forall T}}
|| S \oland f(S_i,T^p_i) - T_i || = || S_i \oland W_c - T_i ||
\label{eq:FFDnet_loss}
\end{equation}

Where $||\cdot||$ can be any error measure ({\em e.g.,} $\mathcal{L}_1$-norm or $\mathcal{L}_2$-norm). We use the smooth huber loss, which is more robust to outliers than $\mathcal{L}_2$-norm and more accurate on inliners compared with $\mathcal{L}_1$-norm, given by  

\begin{equation}
 L^H(T,\hat{T}) = \left\{
                \begin{array}{ll}
                  \frac{1}{2}(T-\hat{T})^2 \quad \quad \textrm{for} \: |T-\hat{T}|< 1, \\
                  (T-\hat{T}) - \frac{1}{2} \quad \: \textrm{otherwise.}
                \end{array}
              \right.
\label{eq:huber}
\end{equation}

The proposed approach enables training without ground-truth FFDs while simultaneously learning to be partial-shape agnostic. During test-time, given a source shape $S$ and a target shape with different parts missing $T^{p_1}, T^{p_2}, \cdots T^{p_n} \in T$ (from test set), FFDnet demonstrates partiality-agnostic-behavior by computing very similar FFDs across for different partialities of the same underlying target (see Figure~\ref{fig:teaser}). We attribute this generalization to the self-supervised nature of the training process.

%Note that if the shapes are full (non-partial) we can optimize for the analytical upper bound (described in Appendix~\ref{sec:optimization}).
\subsection{FFD Regularization}
Estimating the FFD without direct supervision warrants FFDnet to falsely conjecture about the possible deformation field. Solely relying on the self-supervised paradigm defined in Equation~\ref{eq:FFDnet_loss} is ill-posed, since the large degree of freedom in FFDs yields wildly different deformations all with very similar cost. Since knowing the true corresponding RGB textures between source and target shapes requires knowing ground truth deformation fields, FFDnet operates solely on binary silhouettes. Specifically, binary silhouettes are problematic since any FFD which deforms source foreground pixels to target foreground pixels, even if parts are completely rearranged, would result in the same loss. Therefore, we propose several smoothness priors which when added as regularization terms increase the cost of unsuitable FFDs.

\subsubsection{Relative Displacement Fields} 
Instead of directly estimating the FFD displacement field, we propose estimating a displacement field that is relative to the preceding value in the grid which when cumulatively summed results in the absolute displacement field. The relative displacement field has nice properties for facilitating penalizing undesirable fields (\emph{e.g.,} enforcing axial monotonicity). 

To illustrate relative sequences, consider a $1$-dimensional n-length \emph{relative} sequence ${{\Delta a = \left(\Delta a_k \right)_{k=1}^n = ( a_1, a_2, a_3, \cdots )}}$. The cumulative sum at the $k^{th}$-element is $ a_k = \sum_{i=1}^k \Delta a_i + b_0$ where $b_0$ is a scalar offset. So the absolute sequence is given by 

\begin{equation}
a = \cumsum(\left( \Delta a_k \right)_{k=1}^n,b_0) = \left( \sum_{i=1}^k \Delta a_i + b_0 \right) _{k=1}^n
\label{eq:cumsum}
\end{equation}

To add the proposed $\cumsum$ layer into the network for training, it easy to see that the derivative is given by

\begin{equation}
\partial a = \left( \sum_{i}^k \partial a_i \right) _{k=1}^n
\label{eq:cumsum_deriv}
\end{equation}

Since $a$ is a 1-dimensional sequence that is derived from cumulatively summing $\Delta a$, we can claim that $a$ is strictly monotonic when $\Delta a > 0$. The resulting 1-dimensional sequence is a bijection

\begin{equation}
k \longmapsto a_k \because a \triangleq \cumsum(\Delta a > 0, \beta) 
\label{eq:cumsum_bij}
\end{equation}

For the case of the 2-dimensional displacement fields, the $\cumsum$ operator sums along each dimension, respectively. It follows that the absolute displacement field is derived from the relative displacement field, along with a learned scalar  $W_c = \cumsum(\Delta W_c, \beta) $. By enforcing strictly positive relative displacement values $\Delta W_c > 0$, we ensure axial monotonicity in the displacement fields. Axial monotonicity means that each axis is monotonically increasing (independent of the opposing axis). Explicitly imposing axial monotonicity encourages smooth warp fields, and decreases the likelihood of flips.

\subsubsection{Identity Penalty}
The relative displacement formulation yields interesting properties for encouraging smoothness, specifically in the form of identity penalty. Note that the absolute identity FFD (non-relative) is given by uniformly spaced grid between $[-1, 1]$. Meaning, $W^I_c$ defined on a $mxm$ sized grid, sweeps in increments of $\delta_m = \frac{2}{m-1}$ such that $[-1, -1 +\delta_m, -1 + 2\cdot \delta_m, \cdots, 1]$ in both dimensions. However, the relative FFD identity $\Delta W^I_c$ simply contains a single scalar ($\delta_m$) for all-entries of the grid $\Delta W^I_c \triangleq \frac{2}{m-1}$. Therefore, we incorporate an additional a cost for deviating from the identity deformation in the form of

\begin{equation}
\lambda \cdot ||\Delta W_c - \delta_m||
\label{eq:id_ffd}
\end{equation}

where $\lambda$ is the parameter used regulate smoothness, and $||\cdot||$ is the same robust huber penalty defined in Equation~\ref{eq:huber}.

\subsection{Unsupervised Training Data}
In a fully supervised setting, the ground-truth correspondences (or FFD) are known, and we can optimize for the correct deformation. Naturally, manual generation of ground-truth correspondences is a cumbersome task and prone to errors. Automatic ground-truth generation (arguably solving the task itself), limits the network to be as good as good as the algorithm utilized, but for partial data. Judging the success of the network by applying the FFD on the input source shape in a self-supervised manner, mitigates the need for large amounts of labeled data.

We use several different types of data for training, considering pairs of source and target shapes to be different instances from the same class. We render lower and upper case (56 classes) for 330 fonts and 2D projections from objects from ShapeNet~\shortcite{shapenet2015}, and split into training and testing data. All silhouettes are merely binary (this paper displays RGB or checkerboard images entirely for the sake of visualization). See a small subset of silhouette instances in figure~\ref{fig:instace_examples}.

\begin{figure}[h]
	%\centering%
\jsubfig{\includegraphics[height=2.5cm]{figures/chair_samples25.png} }
	%{subtitle1}%
    \;
 \jsubfig{\includegraphics[height=2.5cm]{figures/H_samples25.png} }
	%{subtitle2}%
    \;
  \jsubfig{\includegraphics[height=2.5cm]{figures/airplane_samples25.png}}
	%{subtitle3}%
    
\caption{Small random subset of the silhouette shape data used for training. Instances from different classes: uppercase H, airplane and chair}
\label{fig:instace_examples}
\end{figure}

At first the set of 300 shapes may seem small, but the number of unique pairs is the number of 2-length permutations (\emph{e.g,} for 300 yields ~90k). Furthermore, the effective number of unique training examples is even larger since it is possible to generate an arbitrarily large amount of partial data. We remove different silhouette elements by randomly selecting the part location, width and height to generate partial data on-the-fly during training. Moreover, the self-supervision in FFDnet facilities several forms of data augmentation that yield in nearly-novel silhouettes. Specifically, we further augment the training set by applying a small scaling in x and y.

\end{comment}

% * <overleaf@hanocka.com> 2017-07-29T13:09:33.170Z:
% 
% > 300
% it's around 300 now, but I found more...
% 
% ^.




